Understanding the Evolution of Blockchain Ecosystems: A Longitudinal Measurement Study of Bitcoin, Ethereum, and EOSIO

The continuing expansion of the blockchain ecosystems has attracted much attention from the research community. However, although a large number of research studies have been proposed to understand the diverse characteristics of individual blockchain systems (e.g., Bitcoin or Ethereum), little is known at a comprehensive level on the evolution of blockchain ecosystems at scale, longitudinally, and across multiple blockchains. We argue that understanding the dynamics of blockchain ecosystems could provide unique insights that cannot be achieved through studying a single static snapshot or a single blockchain network alone. Based on billions of transaction records collected from three representative and popular blockchain systems (Bitcoin, Ethereum and EOSIO) over 10 years, we conduct the first study on the evolution of multiple blockchain ecosystems from different perspectives. Our exploration suggests that, although the overall blockchain ecosystem shows promising growth over the last decade, a number of worrying outliers exist that have disrupted its evolution.

==> Section-V-DApp.tex <==
\section{DApp Ecosystem}
\label{sec:dapp}
Smart contract has been first used in blockchain in Ethereum, in which the ability of interacting among smart contracts makes the appearance of DApp possible. Moreover, the resource model of EOSIO encourages the emergence of gambling and DeFi DApp that requires frequent money transfer or contract invocation.
Therefore, based on the $MTG$ and $CIG$ for both above platforms and the DApp information we collected (see \S\ref{sec:study-design:data-collection}), we extracted all the DApp-related traces for each month.
Specifically, if the $label$ attribute of either one of the two nodes of a trace contains a DApp's information, we regard this trace as a DApp-related trace and classify it into the corresponding category by $label$.
Then, we utilized these DApp-related traces to construct a series of $MTG$ and $CIG$ like the methodology we adopted in \S\ref{sec:blockchain-evolution}.
In this section, we would first give an overview of the DApp information we collected. Then, we would picture the overall ecosystem of DApps in Ethereum and EOSIO. Finally, we will pick out the DApp-related traces belonging to the two most representative categories: gambling and DeFi, to explore some interesting findings.

\subsection{DApp Overview}
\label{sec:dapp:overview}
As we mentioned in \S\ref{sec:study-design:data-collection}, we have collected the largest-ever dataset on DApp information on both Ethereum and EOSIO. Moreover, we made a great effort on verifying the correctness of the DApps belonging categories.
Table~\ref{table:dapp} shows brief descriptions of the categories which we have adopted, as well as the number of the corresponding DApps.

\begin{table}[tbp]
\caption{The description of categories, as well as the number of corresponding DApps.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcc}
\toprule
\textbf{Category}  & \textbf{Desc.} & \textbf{\#Ethereum (\#Addr)} & \textbf{\#EOSIO (\#Addr)} \\
\midrule
\textbf{DeFi}      & Financial products that directly build on blockchain technology     & 73 (4,386)                   & 8 (23)                    \\
\textbf{Exchange}  & A palace allows user to exchange fiat currency and cryptocurrency   & 162 (328)                    & 40 (96)                   \\
\textbf{Finance}   & DApps that are related to financial product                         & 95 (316)                     & 10 (19)                   \\
\textbf{Gambling}  & It requires players to invest tokens and may return more            & 377 (1,107)                  & 372 (1,052)               \\
\textbf{Game}      & All non-gambling games, e.g., collectible card games                & 1,109 (5,126)                & 97 (163)                  \\
\textbf{High-Risk} & Applications that are often characterized by Ponzi schemes          & 335 (453)                    & 47 (68)                   \\
\textbf{Platform}  & On which users can develop or deploy other applications or services & 72 (158)                     & 16 (34)                   \\
\textbf{Social}    & Social applications (like dating) that adopt blockchain technology  & 76 (134)                     & 20 (31)                   \\
\textbf{Token}     & Unofficial token issued on the blockchain platform                  & 854 (909)                    & 3 (4)                     \\
\textbf{Tool}      & Provide users with convenient and efficient tools                   & 139 (301)                    & 38 (65)                   \\
\textbf{EIDOS}     & A malicious but phenomenal DApp in EOSIO                            & -                            & 1 (1)                    \\
\bottomrule
\end{tabular}%
}
\label{table:dapp}
\end{table}

As we can see from Table~\ref{table:dapp}, in EOSIO, the number of gambling DApp has absolutely dominated the EOSIO's DApp, and it was also popular in Ethereum. However, game DApps in Ethereum has occupied larger share, around 38.78\% addresses are related to game DApps. Moreover, 73 DeFi DApps in Ethereum has accounted for about one third of DApp addresses. We speculate that the reason for this phenomenon is that decentralized exchange needs different smart contracts to act as different trading pairs. For example, Uniswap~\cite{}, a well-known decentralized exchange, has 410 contract address according to our dataset.
Last but not least, we can not omit the EIDOS DApp in EOSIO, which receives EOS tokens transferred from any accounts, and then immediately returns all EOS tokens and attaches a certain amount (independent of the number of the transferred EOS tokens) of EIDOS tokens. Since EIDOS tokens can be circulated on the secondary market and have a certain value, users can transfer EOS to this type of DApps at a very high frequency and get profit with no cost. To this end, EIDOS has caused huge amount of spam transactions, which will be detailed in \S\ref{sec:dapp:evolution} and \S\ref{sec:abnormal-behaviors:case-study:EIDOS}.


\subsection{Overall Evolution}
\label{sec:dapp:evolution}
After extracting all the DApp-related traces, we analyzed the percentage of $T_m$ and $T_c$ belonging to different DApp categories, which are shown in Fig.~\ref{fig:dapp-mtg} and Fig.~\ref{fig:dapp-cig}, respectively.

\subsubsection{DApp's Money Transfer}
\label{sec:dapp:evolution:mtg}
From the perspective of money transfer, we can easily observe from Fig.~\ref{fig:dapp-mtg-eos} that gambling DApp dominates EOSIO's DApp ecosystem overwhelmingly. To be specific, from the third month of its very beginning, i.e., August, 2018, the gambling DApps were continuously accounting for more than 90\% of $T_m$ in the corresponding months. Astonishingly, the number has reached up to the highest point in 2018-11: 99.01\%.
However, from 2019-11, the EIDOS began to dominate the whole ecosystem by an overwhelming margin, around 99.39\% in November 2019.
Except for these two categories, we can see exchanges also play an important role in EOSIO's ecosystem. Prior to 2019-11, exchange-related transfers began to become more active, which indicates users began to buy and sell EOS tokens more frequently. According to our statistics, the most active exchanges are: DEXEOS~\cite{}, WhaleEx~\cite{}, Findex~\cite{} and Newdex~\cite{}.
Also, we can see 79.51\% of $T_m$ was related to game DApps only in 2018-07. After a comprehensive analysis, we found it was caused by a game DApp called PumpDumpWars~\cite{}, \he{which is a xxx}.

From Fig.~\ref{fig:dapp-mtg-eth}, we can see that platform DApps (a mining pool called Dawrfpool~\cite{}) took up all the initial market share till mid-2017. However, its absolute number was actually relatively small. According to the statistics, it had took up at most 20.22\% of all $T_m$, which happened in 2016-02 (see Fig.~\ref{fig:no-dapp}).
In addition, we can see a spike of tool DApps in mid-2017. It is a DApp called Ethereum Name Service (ENS)~\cite{}, which provides services that exchange between the abstract Ethereum addresses to human-readable strings.
Moreover, two obvious spikes related to game and gambling DApps in December 2017 and August 2018 can be easily noticed, which are resulted from the prosperity of CryptoKitties~\cite{} and Last Winner~\cite{}.
DeFi has started to flourish from the beginning of 2018, and became more and more important. At meanwhile, gambling DApps also started to capture the market of game DApps. We think the reason may be the popularity of Fomo3D~\cite{}, a phenomenal gambling DApp in Ethereum at mid-2018, and prosperity of gambling DApps on EOSIO platform, which both contributed to the prevalence of gambling DApps.

% non-dapp
Moreover, Fig.~\ref{fig:no-dapp} illustrates the percentage of non-DApp-related traces in corresponding months, which shows a significant difference between DApp ecosystems of Ethereum and EOSIO.
We can easily observe that more than three quarters of $T_m$ in EOSIO was related to DApps at most time. But instead in Ethereum, less than one quarter of $T_m$ was related to DApps.

\begin{figure}
     \centering
     \begin{subfigure}[t]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/dapp-mtg-eth.pdf}
         \caption{Ethereum}
         \label{fig:dapp-mtg-eth}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[t]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/dapp-mtg-eos.pdf}
         \caption{EOSIO}
         \label{fig:dapp-mtg-eos}
     \end{subfigure}
        \caption{Percentage of different categories of DApps in terms of money transferring.}
        \label{fig:dapp-mtg}
\end{figure}

\textbf{\textit{Insight:}} In terms of DApp-related $T_m$, gambling DApps nearly dominated the EOSIO's DApp ecosystem until the appearance of EIDOS. Along with the prosperity of gambling DApps, exchanges also play a vital role in EOSIO. Moreover, Except for the beginning four months, no less than 80.64\% of $T_m$ was related to kinds of DApps.
Compared to EOSIO, the ecosystem of Ethereum's DApps was less active. However, there did not exist a certain category of DApps that dominated a period within Ethereum. In other words, The rise and fall of percentage of various categories of DApps reflected the diversity of this ecosystem.


\subsubsection{DApp's Contract Invocation}
\label{sec:dapp:evolution:cig}
Fig.~\ref{fig:dapp-cig} reveals the contract invocation behavior related to DApps on both platforms. 
Specifically, Fig.~\ref{fig:dapp-cig-eos} reveals the DApp-related $T_c$ in EOSIO. Compared with the money transfer in EOSIO (see Fig.~\ref{fig:dapp-mtg-eos}), the biggest distinction is the appearance of traces related to social and platform DApps in 2018-07 and almost whole year of 2019, respectively. According to our statistics, we figured out the social DApp are ChallengeDapp~\cite{} and KARMA~\cite{}, and the platform DApp is pornhashbaby~\cite{}, which provides the pornography storing and sharing service but was shut down in November 2019.

Similarly, the DApp-related $T_c$ in Ethereum (see Fig.~\ref{fig:dapp-cig-eth}) are more complicated than the money transfer's.
We can easily observe that the number of $T_c$ categorized as token DApps increased suddenly. That is because we regard all the unofficial token transfers (see category \textbf{Token} in \S\ref{sec:dapp:overview}) in Ethereum as contract invocation.
Except the emergence of token DApps, the DeFi has been capturing more and more market. As DeFi requires frequently interactions between DeFi DApps, which pushed the number higher than ever.
Moreover, we can observe that the gambling-related $T_c$ has occupied lots of shares which original belonged to platform DApps (mainly Dawrfpool) before mid-2017. We think the reason is these gambling DApps accepted unofficial tokens as betting from players, which would only increase the number of $T_c$.
Additionally, we can obtain some abnormal spikes: `tool' in 2017-05, `gambling' in 2019-09, and `game' in 2019-11, which are caused by ENS, Fairwin~\cite{} (a well-known but transitory gambling DApp), and Gods Unchained TCG~\cite{} (a collectable trading cards game, like the CryptoKitties), respectively.

Talking about the percentage of non-DApp $T_c$, it has completely different characteristics from that of money transfer. 
Specifically, in Ethereum, the percent of non-DApp $T_c$ has dropped to nearly 50\% compared with 80\% of non-DApp $T_m$ at the same time period. For EOSIO, however, the opposite is true.
The main reason for this phenomenon we believe is that traces related to unofficial tokens transfer is more active in Ethereum compared to Ether, while the opposite is true in EOSIO.

\begin{figure}
     \centering
     \begin{subfigure}[t]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/dapp-cig-eth.pdf}
         \caption{Ethereum}
         \label{fig:dapp-cig-eth}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[t]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/dapp-cig-eos.pdf}
         \caption{EOSIO}
         \label{fig:dapp-cig-eos}
     \end{subfigure}
        \caption{Percentage of different categories of DApps in terms of contract invocation.}
        \label{fig:dapp-cig}
\end{figure}

\begin{figure}[tbp]
\centerline{\includegraphics[width=0.7\columnwidth]{images/no-dapp.pdf}}
\caption{Percentage of non-DApp money transferring and contract invocation traces in Ethereum and EOSIO.}
\label{fig:no-dapp}
\end{figure}


\textbf{\textit{Insight:}} In EOSIO's DApp ecosystem, the characteristics of $T_c$ is similar to that of $T_m$. However, the pornography platform occupied a certain share till its close in November. Comparing with $T_m$, the percentage of DApp-related $T_c$ is a little bit lower, but still higher than that of Ethereum.
Ethereum still illustrated the diversity mentioned in \S\ref{sec:dapp:evolution:mtg}. However, the tokens' related transfer has accounted for a large proportion, and DeFi has been dominating the ecosystem, reaching 66.38\% in March 2020. Moreover, the game DApps, which initiated and received lots of $T_c$ to perform the game logic, can not be neglected from the late-2017 till the time of writing.


\subsection{Gambling \& Defi DApps}
\label{sec:dapp:defi-gambling}
We decided to extract the sub-figures of $MTG$ and $CIG$ that are composed of all the traces related to gambling and DeFi DApps respectively to delve deeper for these two representative categories.

\subsubsection{Gambling Ecosystem}
\label{sec:dapp:defi-gambling:gambling}
Gambling DApps has emerged since the very beginning of these two platforms and always holds a certain of shares of DApp ecosystems, especially in EOSIO (see \S\ref{sec:dapp:evolution}). Therefore, we firstly characterized sub-graphs related to gambling DApps.

\begin{figure}
     \centering
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/gambling-basic-mfg-node.pdf}
         \caption{$MTG$}
         \label{fig:gambling-basic-mfg-node}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/gambling-basic-cig-node.pdf}
         \caption{$CIG$}
         \label{fig:gambling-basic-cig-node}
     \end{subfigure}
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/gambling-basic-mfg-trace.pdf}
         \caption{$MTG$}
         \label{fig:gambling-basic-mfg-trace}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/gambling-basic-cig-trace.pdf}
         \caption{$CIG$}
         \label{fig:gambling-basic-cig-trace}
     \end{subfigure}
        \caption{Number of nodes and traces within sub-$MTG$ and sub-$CIG$ that are related to gambling DApps.}
        \label{fig:gambling-basic}
\end{figure}

Fig.~\ref{fig:gambling-basic} shows the number of nodes included in each months' gambling-related $MTG$ and $CIG$, as well as the number of traces. 
We can see that gambling DApps were much more popular in EOSIO in terms of both absolute number and relative percentage at least prior to November 2019.
To be specific, though gambling DApps has emerged earlier in Ethereum and held a certain of market (see Fig.~\ref{fig:dapp-cig-eth}), there was only 10.84\% of $T_c$ in April 2017 related to the gambling DApps as shown in Fig.~\ref{fig:gambling-basic-cig-trace}, which is the maximum point in the earlier stage of Ethereum.
In late-2018, gambling DApps related $T_c$ has occupied up to 88.53\% in EOSIO in October 2018. The percentage for $T_m$ went even higher, reached up to 94.67\% at the same month shown in Fig.~\ref{fig:gambling-basic-mfg-trace}.
Interestingly, we can see three strange spikes in Fig.~\ref{fig:gambling-basic-mfg-node}: August 2018 and May 2019 in Ethereum, April and June in 2019 in EOSIO. For Ethereum, the reason lies behind were the Last Winner~\cite{} and CoinGathernator~\cite{}.
However, in EOSIO, it is because the \textit{spam advertisements} initiated from some gambling DApps. To be specific, the content of advertisements was embedded in the transaction in which it carries a tiny amount of EOS to attract the players' attention. We can see from Fig.~\ref{fig:gambling-basic-mfg-trace}, the few pieces of advertisement did not have ability to change the whole ecosystem but covered lots of users in that month, i.e., 61.53\% and 73.95\% of users who included in $MTG_{eos}^{2019-04}$ and $MTG_{eos}^{2019-06}$, respectively.

 \begin{figure}
     \centering
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/gambling-alpha-mfg.pdf}
         \caption{$MTG$}
         \label{fig:gambling-alpha-mfg}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/gambling-alpha-cig.pdf}
         \caption{$CIG$}
         \label{fig:gambling-alpha-cig}
     \end{subfigure}
        \caption{$\alpha$ of indegree/outdegree distribution within sub-$MTG$ and sub-$CIG$ that are related to gambling DApps. Blue lines are for Ethereum, and red lines are for EOSIO.}
        \label{fig:gambling-alpha}
\end{figure}

\begin{figure}[tbp]
\centerline{\includegraphics[width=0.5\columnwidth]{images/gambling-pearson-eth.pdf}}
\caption{R of indegree and outdegree distribution in Ethereum related to gambling DApps.}
\label{fig:gambling-pearson-eth}
\end{figure}

When we delve deeper to investigate the change of $\alpha$ of indegree/outdegree distributions, we can easily observe from Fig.~\ref{fig:gambling-alpha-cig} that the $\alpha$ of outdegree distribution in Ethereum is much more higher than that of indegree distribution. Combining with the relative small number of $T_c$ in gambling DApps (see Fig.~\ref{fig:gambling-basic-cig-trace}), it is easy to draw conclusion: a few small number of gambling DApps in Ethereum has received almost all the gambling related $T_c$, and the players are dispersed among the Ethereum which leads to such a small $\alpha$ of outdegree distribution.
Moreover, Fig.~\ref{fig:gambling-pearson-eth} depicts the R between indegree and outdegree distribution in Ethereum in terms of gambling DApps. During the most active period of gambling DApps in Ethereum, i.e., mid-2017, the R of $CIG$ even shows a negative correlation, which indicates that those gambling DApps who received lots of $T_c$ hardly initiated another $T_c$.

Recall the appearance of Fairwin in September 2019 which leads to conspicuous spikes in Fig.~\ref{fig:dapp-cig-eth} and Fig.~\ref{fig:gambling-alpha-cig}. Within our analysis, the percentage of $T_c$ has reached up to 25.81\%, while the value of $\alpha$ of indegree distribution was -4.988. Moreover, the R of $CIG$ and $MTG$ were opposite, which are -0.078 and 0.997, respectively.
These values jointly indicates this gambling DApp in Ethereum centralized more than one quarter of $T_c$ in that month. However, the number of scattered players are so high (see the spike in Fig.~\ref{fig:gambling-basic-mfg-node} and Fig.~\ref{fig:gambling-basic-cig-node}) to pull the $\alpha$ down. In addition, the two values of R indicate that Fairwin did not initiated much $T_c$ but a high number of $T_m$.

\textbf{\textit{Insight:}} Gambling DApps dominated the EOSIO ecosystem, though some of the high coverage are due to the spam advertisements behavior. Contrary to the long-term prosperity of gambling DApps in EOSIO, Ethereum's popular ones are more in a transitory situation. In other words, some killer gambling DApps emerged and attracted lots of attention from players in Ethereum, but they disappeared suddenly.

\subsubsection{DeFi Ecosystem}
\label{sec:dapp:defi-gambling:defi}
DeFi, as the most popular category of DApps now, has attracted lots of investors, as well as the malicious users. For example, Lendf.me, a famous lending platform based on decentralized finance technology, has been attack in April 2020, which leads to more than 25 million USD financial loss~\cite{}.
% https://www.zdnet.com/article/hackers-steal-25-million-worth-of-cryptocurrency-from-uniswap-and-lendf-me/
Moreover, from Fig.~\ref{fig:dapp-mtg-eth} and Fig.~\ref{fig:dapp-cig-eth}, we can easily observe the liveness of DeFi DApps. Thus, in this section, we would explore the characteristics of DeFi DApps in Ethereum and EOSIO.

\begin{figure}
     \centering
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/defi-basic-mfg-node-scale.pdf}
         \caption{$MTG$}
         \label{fig:defi-basic-mfg-node}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/defi-basic-cig-node.pdf}
         \caption{$CIG$}
         \label{fig:defi-basic-cig-node}
     \end{subfigure}
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/defi-basic-mfg-trace-scale.pdf}
         \caption{$MTG$}
         \label{fig:defi-basic-mfg-trace}
     \end{subfigure}
%     \hfill
     \begin{subfigure}[t]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/defi-basic-cig-trace.pdf}
         \caption{$CIG$}
         \label{fig:defi-basic-cig-trace}
     \end{subfigure}
        \caption{Number of nodes and traces within sub-$MTG$ and sub-$CIG$ that are related to DeFi DApps.}
        \label{fig:defi-basic}
\end{figure}

Fig.~\ref{fig:defi-basic} shows the number of related nodes, $T_m$, and $T_c$ in $MTG$ and $CIG$.
We can easily observe that, DeFi related traces are more classified into the $CIG$.
As we have observed in Fig.~\ref{fig:dapp-mtg-eos} and Fig.~\ref{fig:dapp-cig-eos}, DeFi was account for a tiny fraction of $T_m$ and $T_c$ in EOSIO: less than 1\% for both types of graphs. However, we can still see three conspicuous spikes in Fig.~\ref{fig:defi-basic-mfg-node} in 2018-11, 2019-05 and 2019-11, respectively. After the manual analysis, we found that the first two spikes were caused by Chintai~\cite{} and EOS REX~\cite{} (resource exchange platform in EOSIO), respectively. However, for November 2019, the number of nodes 7,366 did not increase too many compared to the preceding month (7,324 nodes in October 2019). Therefore, we think this spike is due to the congestion resulted by EIDOS.
As for Ethereum, steep growth trends in both $MTG$ and $CIG$ can be observed. Except the trough in late-2019, which is caused by the decline of coverage of USDT (a well-known stable coin in Ethereum), DeFi has accounted for 34.62\% of $T_c$ in March 2020 and still kept an upward tendency. Compared to contract invocation, DeFi led to less money (Ether) transfer, however, it still account for about 7\% of $T_m$ at the same time.

\begin{figure}[tbp]
\centerline{\includegraphics[width=0.5\columnwidth]{images/defi-alpha-cig.pdf}}
\caption{$\alpha$ of indegree/outdegree distribution within sub-$CIG$ that are related to DeFi DApps.}
\label{fig:defi-alpha-cig}
\end{figure}

As the DeFi DApps are mainly interacted with each other in $CIG$, we only measured the $\alpha$ of indegree/outdegree distribution in $CIG$ for both platforms as shown in Fig.~\ref{fig:defi-alpha-cig}.
The point in 2019-01 is obvious, the $\alpha$ of outdegree and indegree distribution moved to opposite directions simultaneously. We think the reason was the appearance of a DeFi called Chintai~\cite{}, which is a platform where users can lend their EOS on the market to earn interest.
Moreover, for both platforms, we can observe an interesting phenomenon: the $\alpha$ of indegree distribution nearly always higher than that of outdegree distribution. This indicates there were several head DeFi DApps that absorbed users' contract invocation requests.
According to our statistics, the most 10 popular DeFi DApps in Ethereum's history and the number of its received $T_c$, as well as the covered users, are shown in Table~\ref{table:top10-defi}.
We can see that, 4 out of top 5 are the stable coins, which provide a relative stable price by some financial measures. The most widely used stable coin is USDT~\cite{}, which has more than 3 million users who have invoked more than 4.3 million pieces of $T_c$.
More than stable coins, exchanges and money markets also appeared in the top 10. Specifically, exchanges here refer to decentralized exchanges (DEX), which utilized smart contracts to automatically perform matchmaking. However, several blogs~\cite{} and previous works~\cite{} have reported and studied the vulnerability existed in DEXes. As for money market, it provides a platform to allow user lends and loans cryptocurrency with it.

\begin{table}[tbp]
\caption{Top 10 DeFi DApps in Ethereum and its corresponding number of $T_c$ and nodes.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccc}
\toprule
                   & \textbf{USDT} & \textbf{USDC} & \textbf{IDEX} & \textbf{PAX} & \textbf{DAI} & \textbf{Oasis} & \textbf{CDP Portal} & \textbf{Uniswap} & \textbf{TUSD} & \textbf{Bancor} \\
\midrule
\textbf{Category}  & \begin{tabular}[c]{@{}c@{}}Stable\\ Coin\end{tabular} & \begin{tabular}[c]{@{}c@{}}Stable\\ Coin\end{tabular} & Exchanges     & \begin{tabular}[c]{@{}c@{}}Stable\\ Coin\end{tabular} & \begin{tabular}[c]{@{}c@{}}Stable\\ Coin\end{tabular} & \begin{tabular}[c]{@{}c@{}}Money\\ Market\end{tabular} & \begin{tabular}[c]{@{}c@{}}Money\\ Market\end{tabular} & Exchanges        & \begin{tabular}[c]{@{}c@{}}Stable\\ Coin\end{tabular} & Exchanges       \\
\textbf{\# $T_c$} & 4,335,452     & 624,793       & 603,680       & 451,442      & 406,847      & 261,888        & 261,423             & 148,544          & 146,433       & 121,159         \\
\textbf{\# Nodes}  & 3,074,449     & 508,592       & 273,815       & 407,656      & 301,911      & 106,761        & 122,859             & 41,131           & 105,198       & 34,501         \\
\bottomrule
\end{tabular}%
}
\label{table:top10-defi}
\end{table}

%\begin{figure}[tbp]
%\centerline{\includegraphics[width=0.5\columnwidth]{images/defi-pearson-cig.pdf}}
%\caption{R between indegree and outdegree within sub-$CIG$ that are related to DeFi DApps for both platforms.}
%\label{fig:defi-pearson-cig}
%\end{figure}

\begin{figure}[tbp]
\centerline{\includegraphics[width=0.5\columnwidth]{images/defi-cc-cig.pdf}}
\caption{The number of WCC and SCC within $CIG$ that are related to DeFi DApps for both platforms.}
\label{fig:defi-cc-cig}
\end{figure}

Fig.~\ref{fig:defi-cc-cig} depicts the number of WCC and SCC related to the DeFi DApps in $CIG$. We can observe that the numbers of SCC in Ethereum were overall higher than EOSIO's. We think this must be due to the frequent interaction between users and DeFi DApps, as the corresponding numbers of WCC were only fluctuating around a relative low level.
%\he{add the number of the largest size of WCC and SCC here, @Weihang}. 
The three spikes in the number of SCC in EOSIO exactly corresponds with the events mentioned in Fig.~\ref{fig:defi-basic-mfg-node}.

\textbf{\textit{Insight:}} DeFi in Ethereum has been being under a flourishing development, some of head DeFi DApps has attracted lots of users who initiate $T_c$ to interact with them. At meanwhile, it did not be developed well in EOSIO, in which only the unabiding DeFi DApps emerged.


\subsection{Summary}
\he{high level summary for this whole section, TBD}







































